SoK: Machine Learning for Misinformation Detection

We examine the disconnect between scholarship and practice in applying machine learning to trust and safety problems, using misinformation detection as a case study. We survey literature on automated detection of misinformation across a corpus of 248 well-cited papers in the field. We then examine subsets of papers for data and code availability, design missteps, reproducibility, and generalizability. Our paper corpus includes published work in security, natural language processing, and computational social science. Across these disparate disciplines, we identify common errors in dataset and method design. In general, detection tasks are often meaningfully distinct from the challenges that online services actually face. Datasets and model evaluation are often non-representative of real-world contexts, and evaluation frequently is not independent of model training. We demonstrate the limitations of current detection methods in a series of three representative replication studies. Based on the results of these analyses and our literature survey, we conclude that the current state-of-the-art in fully-automated misinformation detection has limited efficacy in detecting human-generated misinformation. We offer recommendations for evaluating applications of machine learning to trust and safety problems and recommend future directions for research.

==> src/02_related_work.tex <==
\section{MOTIVATION}
\label{sec:motivation}

The detection of misinformation and ``influence operations'' (IOs) is a topic of convergent interest for security, social science, and NLP researchers. Methods developed in recent years for the detection of influence operations (e.g., astroturfing, coordinated misinformation campaigns) resemble techniques previously employed by security researchers for the detection of botnets, advanced persistent threats (APTs), and malware \cite{milajerdi2019holmes,king2006subvirt,stone2009botnet}. As such, we believe that the security community is uniquely well-positioned to shepherd the responsible development of misinformation detection methods. In addition, misinformation research stands to benefit a good deal from the formal structure of security research methodology: In a survey study from 2022, Mirza et al. found that human fact-checkers and journalists would likely benefit from rigorous threat modeling practices similar to those found in security literature \cite{mirza2023tactics}. 

We situate our work within existing literature that describes content moderation operations on social media platforms. Though Twitter and Facebook have previously advertised human-in-the-loop processes for automatically flagging potentially misinformative posts for manual vetting by third-party fact-checking organizations, criteria for deploying tiered responses and seeking human intervention are murky \cite{fb_third_party}. Furthermore, evidence from the leaked Facebook Files suggests that automated content moderation methods rely heavily on proxy signals (e.g., text sentiment and sharing patterns) for identifying misinformation on the platform; as a result, automated approaches are generally employed for first-line detection of putative rumoring narratives, with the burden of actual fact verification falling to human moderators \cite{facebook_files_2021}.

==> src/03_methods.tex <==
\section{PRELIMINARIES}
\label{sec:preliminaries}

\textbf{Definitions.} In the absence of agreed-upon definitions of \textit{misinformation, disinformation, malinformation,} and \textit{influence operations}, we refrain from advancing singular definitions of the same. Instead, for each paper we review, we consider the paper authors' working definitions of these terms (if such definitions are provided) and evaluate model performance with respect to the definitions set forth \cite{wu_misinformation_2019,gelfert_fake_2018,haiden_definitional_2018,klein_fake_2017,tandoc_defining_2018}. We discuss misinformation research's definitional problem in greater detail in~\Cref{sec:discussion}. Within our corpus, we also include information that is transparently false, but not intended to mislead: satire, parody, and spoofs.  We limit our analysis to English-language misinformation.\footnote{We acknowledge that the nature of misinformation narratives and misinformation spread varies with language and geography.} We note that \textit{disinformation} is commonly used to refer to incorrect information written with the intent to deceive, while \textit{misinformation} refers to incorrect information in general; for the sake of completeness and concision, we refer to intentionally \textit{and} unintentionally false information as \textit{misinformation} for this work. We occasionally use \textit{false rumors,} \textit{false news,} \textit{false information}, and \textit{misinformative news} interchangeably, but avoid \textit{fake news}, a politically charged term. We use ``influence operations'' (IOs) or ``coordinated campaigns'' in our discussion of collaborative attempts to disseminate misinformation across networks.

\textbf{Feasibility of detection.} Most of the work we review presupposes that automated detection of misinformation is possible at all. We note that this is, in itself, a strong assumption to make: Published work in psychology, linguistics, and philosophy of language has previously called into question the feasibility of using semantic and syntactic features to determine the veracity of text statements and the usefulness of binary true/false classifications of information, particularly in the absence of unified definitions of misinformation, disinformation, and information \cite{soe_2017,vrij_pitfalls_2008}. On the other hand, some researchers maintain that misinformative texts are characterized by indelible ``fingerprints'' that distinguish them from non-misinformative texts: for instance, emotional language and reduced lexical diversity \cite{amado_undeutsch_2015,carrasco_2022}. We use this debate to motivate our discussion of non-textual feature sets for misinformation detection. 

\textbf{Taxonomies.} Through an iterative process of reading and inductive coding of our papers, we develop a taxonomy of five ``information scopes.'' As we read each paper in our corpus, we noted the \textit{operative unit} of misinformation detection for the classifier or method described---the smallest semantic or organizational unit of information that the method attempted to classify as true or false---and sorted each paper into emergent categories. Our final taxonomy comprises five information scopes: \textbf{claims, news articles, social media accounts, networks, and websites.} We consider these scopes \textit{in the context of} online services---e.g., evaluation of news articles and websites whose links might be posted to a social media platform. We note three principle approaches to misinformation detection: \textbf{claim verification, detection of language signals,} and \textbf{analysis of propagation patterns}. We also note the types of features included in each model's feature set, and sort observed feature sets into five categories: \textbf{textual, network-based, infrastructural, user- or author credential-based,} and \textbf{multimodal features,} comprising two or more features from the other four categories. We also note performance and accuracy scores of published methods, if authors report this information. Additional details about our corpus construction and paper coding process can be found in~\Cref{sec:analysis}. 

\textbf{ML critiques.} We adopt the terminology and taxonomies of previous work in our examination of ML errors \cite{kapoor_2022, kaufman_leakages_2012, arp_ml_2022}. In the context of data mining, Kaufman et al. define \textit{leakage} as ``the introduction of information about the target of a data mining problem that should not be legitimately available to mine from'' \cite{kaufman_leakages_2012}. Here, we examine other, related design errors in the context of ML-based methods, including those described by Kapoor and Narayanan (their work includes dependencies and duplicates in datasets, temporal leakage, and poor feature selection within a taxonomy of ML design errors) \cite{kapoor_2022}. In general, these errors lead to inflated model performance in an experimental setting and underperformance in real-world deployments. Though the precise nature of these errors varies by dataset, information scope, and choice of model, we broadly categorize them as errors related to \textbf{dataset curation, feature set selection} and \textbf{model evaluation}. Concise visual summaries of our text corpus and all taxonomies discussed in this section are available in our Appendix. 




==> src/05_rep.tex <==
\section{Replication Studies}
\label{sec:rep_studies}

We conduct replicability and reproducibility studies on three different papers within our corpus at the article, account, and whole website scopes. These works are highly representative of their respective scopes: Nasir et al. \cite{nasir_fake_2021} (\Cref{sec:article_rep}) train a neural network on corpora of true and misinformative news articles; Saeed et al. \cite{saeed2022trollmagnifier} (\Cref{sec:trollmagnifier}) use published lists of trolls to infer the presence of other troll accounts on Reddit; and Baly et al. \cite{baly_predicting_nodate} (\Cref{sec:baly_rep}) examine a multimodal feature set comprising infrastructure, content, and network-based features in order to infer whole-site credibility. For each work, we evaluate replicability and generalizability (\textcolor{blue}{RQ3}). Where possible, we 1) replicate reported results; 2) inspect datasets for potential dependencies; 3) perform ablation analyses to understand individual feature performance; and 4) test on current data. 

Toward understanding the reproducibility of existing detection methods (\textcolor{blue}{RQ3}), we conducted replication analyses of a selection of published methods in our corpus; where necessary, we contacted paper authors to request access to data and code. We describe our methodology for both of these processes in this section.

\textbf{Paper selection criteria and author outreach.} We sorted our full text corpus by information scope. Within each scope, we sorted papers in order of decreasing citation count. We then proceeded as follows:

\begin{enumerate}[nolistsep]
    \item[1.] We attempted to source the full methods and datasets for the most cited paper within each information scope.

    \item[2.] If we were unable to find this information during an independent web search, we reached out to the paper's lead author(s) to request access.

    \item[3.] If this request was unsuccessful---if the author did not respond, or confirmed that the dataset or code was no longer available---we returned to step 1 for the next most highly-cited paper in our corpus within that scope.
\end{enumerate}  

\textbf{Replication analyses.} In order to reproduce results published in a selection of papers and perform cross-cutting analyses on out-of-domain and out-of-sample datasets, we conduct a series of replication analyses on a subset of papers. We chose representative methods from disparate information scopes, and which consider a variety of different feature types. We reproduced results reported in each paper on the datasets mentioned therein, contacting authors when necessary to obtain datasets and code. We evaluated reproducibility and generalizability as follows:


\begin{itemize}[nolistsep]

    \item \textbf{Reproducibility.} We reproduce published results with code and data reported in the original publication. We evaluate availability of code and data and, where possible, compare our analysis outcomes with those reported in the original paper (\textcolor{blue}{RQ3}). 

    \item \textbf{Explainability.} Toward understanding the contributions of specific feature types to overall classifier performance, and why certain approaches work (or don't work), we perform feature ablation studies when appropriate. 

    \item \textbf{Replicability and generalizability.} Model perfor-mance on novel datasets will be useful for determining the generalizability of existing detection methods to different contexts (\textcolor{blue}{RQ4}). For models that were explicitly tested on specific misinformation narratives (e.g., 2020 stolen election narratives), on specific timeframes, or on specific types of misinformation (e.g., parody, satire), we develop current datasets to test method performance on diverse information domains. As much as possible, we attempt to imitate real world contexts.
\end{itemize}

\textbf{Ethical Considerations.} Datasets used for this work were already publicly available or were obtained with permission from study authors. Our outreach study was approved by our institutional review board.

%--------------------------------------------------------------

\subsection{Detection of suspicious language}
\label{sec:article_rep}
We reproduced results from a study published in 2021 by Nasir et al \cite{nasir_fake_2021}. The authors propose a neural net-based approach to the classification of \textit{news articles}. The method employs a hybrid deep learning model that combines convolutional and recurrent neural networks for the classification of real and fake news. The authors report results for tests on two datasets: the ISOT dataset (45,000 news stories, equally distributed across true and false categories, as labeled by PolitiFact) and the FA-KES dataset (804 news stories about the Syrian war, 426 true and 376 false) \cite{isot, fa_kes}. We were able to replicate original paper results and run the method on updated datasets of news articles. Motivated by the prevalence of methods trained on few- or single-source datasets in the article scope, we test possible dependencies related to journalistic house style, as \textit{all true articles in the Nasir et al. training corpus were sourced from Reuters.}


\textbf{Reproducibility of published results.}
Both ISOT and FA-KES are readily available online, and we were able to run the original method of Nasir et al. without issue \cite{isot,fa_kes}. The method code was not publicly available online (the authors sent us their code base after we emailed them a request for access). Weights and parameters for their trained model are published in the original paper \cite{nasir_fake_2021}. We were able to reproduce results originally reported in their published paper (see ISOT-\texttt{original} and FA-KES-\texttt{original} in Table~\ref{tab:nasir}). 


\textbf{House style as a confounder.} To investigate house style as a possible confounder for misinformation detection, we excerpted 100 articles from both Reuters and The New York Times, two news outlets with distinctive (and different) reporting styles. We randomly selected these articles from both outlets' RSS feeds in May 2023. We sourced articles for both corpora from the following verticals: U.S. and world politics, economics, science, and entertainment. Excerpt lengths ranged from 100 to 300 words. These corpora, each comprising 100 true news stories, are labeled ``Reuters-\texttt{original}'' and ``NYTimes-\texttt{original}'' in Table~\ref{tab:nasir}.

\begin{table}[!t]
\small
\centering
\def\arraystretch{1.3}
\begin{tabular}{llrrr}%
\toprule
\textbf{Dataset (size)} & \textbf{Features} & \textbf{Acc.} & \textbf{FPR} & \textbf{FNR}\\
\midrule
\multirow{2}{2cm}{ISOT (45,000)} & 
        \texttt{original} & 0.995 & 0.00 & 0.00 \\    
    &   \texttt{scrubbed} & 0.987 & 0.01 & 0.00 \\ 
\midrule
FA-KES (804) & \texttt{original} & 0.521 & 0.151 & 0.843 \\ 
\midrule
\multirow{2}{2cm}{Reuters (100)} & 
        \texttt{original} & 0.727 & 0.71 & -- \\ 
     &  \texttt{modified} & 0.507 & 0.02 & 1 \\
\midrule
\multirow{2}{2cm}{NYTimes (100)} &
         \texttt{original} &  0.673 & 0.705 & -- \\ 
       & \texttt{modified} &  0.492 & 0.735 & 0.286 \\ 
\midrule
ChatGPT (250) & 
         \texttt{original} & 0.939 & 0.02 & -- \\
\bottomrule
\end{tabular}
\caption{Replication analysis of Nasir et al. (2021). We tested the method of Nasir et al. on both datasets discussed in the original paper, and on novel datasets from Reuters and The New York Times \cite{nasir_fake_2021}.} 
\label{tab:nasir}
\end{table}

We then selectively edited 50\% of the news articles within each corpus. We changed proper nouns, negated verbs, and altered reported statistics so that the factual content of these articles was no longer accurate but house style and tone were preserved. We call these altered text corpora ``Reuters-\texttt{modified}'' and ``NYTimes-\texttt{modified}'' in Table~\ref{tab:nasir}. The classifier had 0.727 accuracy on Reuters-\texttt{original} and 0.673 accuracy on NYTimes-\texttt{original}; this difference is not significant (\textit{p} > 0.05). Additionally, the classifier had about 0.50 (random) accuracy on both modified datasets. The classifier's false positive and false negative rates on modified and original Reuters and NYTimes corpora tell a more interesting story, however: Overwhelmingly, \texttt{false} NYTimes articles were classified as \texttt{true} (FPR = 0.02 and 0.735 for Reuters-\texttt{modified} and NYTimes-\texttt{modified}, respectively), while all \texttt{true} Reuters articles were classified as \texttt{false} (FNR = 1 and 0.286 for Reuters-\texttt{modified} and NYTimes-\texttt{modified}, respectively). These results indicate that the classifier was significantly more conservative in its assignment of \texttt{true} labels for the Reuters dataset than it was for the NYTimes dataset; additionally, \textit{within} each modified corpus, the classifier did not effectively differentiate between true and untrue news articles. We did not investigate the stylistic features of each corpus that might have produced (anti-)conservative label distributions; for this work, however, it is sufficient to note that classifier performance in an adversarial setting was no better than random, and that house style appears to have a significant impact on classifier sensitivity to misinformative texts. 


%------------------trolls/networks---------------------

\subsection{Detection of suspicious accounts}
\label{sec:trollmagnifier}
 We reproduce results from a study published in 2022 by Saeed et al. \cite{saeed2022trollmagnifier}. In summary, the authors propose a method, called TrollMagnifier, for the identification of Reddit accounts that exhibit troll-like behaviors. Like all other account-scoped methods we analyze in the security literature, TrollMagnifier is trained on posting and reply statistics for non-troll and known Russian troll accounts (as identified by Reddit) \cite{saeed2022trollmagnifier}.

\textbf{Reproducibility of published results.} Study authors provided us with pre-processed datasets and classifier code upon email request. The full Reddit Pushshift dataset is freely available online \cite{baumgartner2020pushshift}. We were able to replicate original paper results using these materials. Original account handles were anonymized; as such, we were unable to manually verify if the accounts identified in the original study appeared to be troll-like. 

\begin{figure}[!t]
\centering
% \makebox[\textwidth]
\makebox[0pt]{\includegraphics[scale=0.56]{images/pdp.pdf}}
\label{fig:saeed_pdp}
\caption{Partial dependence plots for each TrollMagnifier feature. Respectively, x1 = ``comments on posts that trolls commented on,'' x2 = ``comments on posts that trolls started,'' x3 = ``direct comment in reply to troll post,'' x4 = ``threaded comment in reply to troll comments on a troll post,'' x5 = ``same title post as troll,'' x6 = ``same title post as troll.''}
\end{figure}

\textbf{Defining ``troll'' accounts.} 
As described in preceding sections (\Cref{sec:systematization_of_literature}, \textit{Accounts}), suspicious account detection suffers from a lack of clear and consistent definitions. Troll accounts cannot be described by degree of automation (while some trolls are bot-like, many others are operated by humans) \cite{cresci_bots_2020} or the nature of the information they spread (this might be political misinformation, ads, or anything in between) \cite{yang2022botometer}; as such, the clearest definition that Saeed et al. implicitly offer is that a troll is an account that exhibits \textit{troll-like behavior}: i.e., interacts with known troll accounts, or appears on the same posts or message threads as these accounts. The authors note in their own work that this approach cannot be used to detect novel trolling behaviors, and requires a seed list of known troll accounts for every new detection task (we note in our discussion of \textit{Account}-scoped data curation practices that the process of identifying these seed accounts is actually a fairly manual one). 

\begin{table*}[!ht]
\footnotesize
    \def\arraystretch{1.4}
    \centering
        \begin{tabular}{lc|cc|cc|cc|cc|cc} 
        \toprule 
%     \hline
Dataset (size) & All features & \multicolumn{2}{p{2cm}}{\centering \texttt{articles} \\ $-$ \hspace{0.75cm} $+$} & \multicolumn{2}{p{2cm}}{\centering \texttt{traffic} \\ $-$\hspace{0.75cm} $+$} &  \multicolumn{2}{p{2cm}}{\centering \texttt{twitter} \\ $-$\hspace{0.75cm} $+$} & \multicolumn{2}{p{2cm}}{\centering \texttt{wikipedia} \\ $-$\hspace{0.75cm} $+$} & \multicolumn{2}{p{2cm}}{\centering \texttt{url} \\ $-$\hspace{0.75cm} $+$} \\
        \midrule
            Full corpus (1066)  & 0.654 & \cellcolor{red!25}0.631 & \cellcolor{teal!70}0.644 & 0.654 & 0.508 & 0.648 & 0.550 & \cellcolor{red!70}0.627 & \cellcolor{teal!20}0.606 & 0.638 & 0.533\\ 
            Med. corpus (400)   & 0.623 & \cellcolor{red!25}0.608 & \cellcolor{teal!70}0.630 & 0.620 & 0.488 & 0.635 & 0.500 & \cellcolor{red!70}0.590 & \cellcolor{teal!20}0.588 & 0.623 & 0.495\\
            Small corpus (250)  & 0.636 & 0.632 & \cellcolor{teal!70}0.596 & 0.632 & 0.524 & \cellcolor{red!25}0.608 & 0.512 & \cellcolor{red!70}0.588 & \cellcolor{teal!20}0.536 & 0.624 & 0.516 \\
            Left bias (398)     & 0.691 & \cellcolor{red!25}0.683 & \cellcolor{teal!20}0.671 & 0.688 & 0.668 & 0.686 & 0.628 & \cellcolor{red!70}0.678 & \cellcolor{teal!70}0.683 & \cellcolor{red!70}0.678 & 0.636\\
            Center (263)   & 0.913 & \cellcolor{red!70}0.810 & \cellcolor{teal!70}0.890 & 0.913 & 0.700 & 0.924 & 0.741 & 0.920 & \cellcolor{teal!20}0.776 & \cellcolor{red!35}0.890 & 0.635\\
            Right bias (405)    & 0.279 & \cellcolor{red!70}0.267 & \cellcolor{teal!70}0.252 & 0.279 & 0.173 & 0.286 & \cellcolor{teal!20}0.230 & 0.274 & 0.205 & \cellcolor{red!35}0.272 & 0.121\\
            \midrule
            Full corpus (1066)  & 0.569 & \cellcolor{red!70}0.523 & \cellcolor{teal!70}0.595 & 0.569 & 0.399 & 0.580 & 0.440 & \cellcolor{red!35}0.552 & 0.538 & 0.577 & 0.373\\ 
            Med. corpus (400)   & 0.563 & \cellcolor{red!70}0.517 & \cellcolor{teal!70}0.580 & \cellcolor{red!35}0.560 & 0.420 & 0.578 & 0.478 & 0.585 & 0.545 & 0.568 & 0.360\\
            Small corpus (250)  & 0.456 & \cellcolor{red!35}0.424 & \cellcolor{teal!70}0.560 & 0.452 & 0.364 & 0.500 & 0.408 & \cellcolor{red!70}0.400 & 0.496 & 0.444 & 0.436 \\
            Low cred. (256)     & 0.590 & \cellcolor{red!70}0.516 & \cellcolor{teal!20}0.633 & \cellcolor{red!35}0.590 & \cellcolor{teal!70}0.641 & 0.629 & 0.445 & 0.609 & 0.633 & \cellcolor{red!35}0.590 & 0.473\\
            Mixed cred. (268)   & 0.407 & \cellcolor{red!70}0.340 & \cellcolor{teal!70}0.474 & 0.407 & 0.0522 & 0.414 & 0.258 & \cellcolor{red!35}0.362 & \cellcolor{teal!20}0.276 & 0.414 & 0.198\\
            High cred. (542)    & 0.349 & \cellcolor{red!70}0.336 & \cellcolor{teal!70}0.408 & 0.349 & 0.255 & 0.369 & 0.271 & \cellcolor{red!35}0.341 & \cellcolor{teal!20}0.316 & 0.351 & 0.218\\
        \bottomrule
        \end{tabular}
    \caption{Replication analysis of Baly et al.: Dropout(--) and feature importance(+) analyses of subsets of Baly et al.'s EMNLP18 dataset, stratified by political leaning and credibility. Most (secondmost) performant feature, as determined by its contribution to overall classifier accuracy on the full feature set, is highlighted in darker (lighter) hues. Fact and bias classification task performances are reported in the top and bottom halves of the table, respectively. }
    \label{tab:baly_ablation}
\end{table*}


\textbf{Implied versus actual data dimensionality.} While the original TrollMagnifier paper strongly implied that the proposed method would leverage networked behaviors to identify troll accounts acting in coordination online, we found that, in actuality, the features under analysis lacked any sort of temporal component and were limited in scope. There were six features in all (described in full in Figure~2), each corresponding to an aggregate engagement statistic. Longitudinal data and timestamps were not available; as such, it was not possible to perform time series analysis. Additionally, account names were not available, which disallowed construction of user graphs. 


\textbf{Feature importance.} In our partial dependence analysis, we find that feature x1---commenting statistics---was the sole feature that consistently produced classification accuracy greater than 0.6 (most other features had accuracy no better than random; two features, x2 and x6, had performance below 0.5). Per our earlier observation that many account-scoped methods target behaviors that are difficult to distinguish from routine online activity, we recommend that feature engineering for account- and network-scoped methods reflect some intuition about the nature of actually suspicious behaviors. Furthermore, the performance of the current feature set---no better than random---suggests that manual classification might be as effective as (or even more effective than) an automated approach that only detects a content-agnostic heuristic. 
%------------------websites---------------------

\subsection{Detection of suspicious websites}
\label{sec:baly_rep}
 We reproduce results from a study published in 2018 by Baly et al \cite{baly_predicting_nodate}. In summary: the authors propose a multimodal approach to the classification of \textit{news websites}. This method is particularly representative of works within this information scope: 50\% of works within this scope use a similar mixed-modalities approach to detecting misinformation websites, and Baly et al. include site-specific feature types, including domain and traffic-based features, in their analysis. Baly et al. analyzed website contents, associated social media accounts, and Wikipedia pages in order to perform two classification tasks: fact and political bias classification. The authors developed a dataset of 1066 websites manually labeled for their political leaning (extreme-left, left, left-center, center, right-center, right, and extreme-right) and degree of credibility (low, mixed, high). These labels were extracted from the Media Bias/Fact Check (MBFC) database \cite{mediabiasfactheck}. We were able to reproduce original study results and perform ablation analyses on existing datasets. We were unable to run the method on an updated dataset, as feature extraction code was not available. 

\textbf{Reproducibility of published results.}
All features extracted for the original analysis were captured in a series of json files. On the one hand, this meant that we were able to readily reproduce results reported in the paper; on the other, this meant that certain elements of the dataset (follower counts on social media, Wikipedia page contents) were out of date. As we did not find documentation in the method repository for re-extraction of these features, we were restricted to conducting our tests on data that were already available. We binned bias labels into \textit{left}, \textit{center}, and \textit{right} categories, as the seven-way taxonomy initially applied to the dataset by MBFC yielded small label classes.  Classifier performance on the resulting three-way bias classification task accords with the results reported by Baly et al. on the same task.

\textbf{Limited model explainability.} 
From our reading of the paper by Baly et al. and our analysis of their code base, we find only limited discussion of feature normalization and the contributions of individual feature sets to overall model performance. The authors trained their model on a set of news articles from an undisclosed source; in order to extract feature vectors for the \texttt{article} feature set for each site in the EMNLP18 dataset, the authors took the unweighted average of 141 GloVe features over the set of retrieved articles (article selection process is not disclosed). There is no discussion of the semantic features included within this set of 141, or of how these features were chosen.  

\textbf{Multimodal features: help or hindrance?} 
We performed an ablation study of the method on the EMNLP18 dataset and analyzed the method's \textit{bias} and \textit{fact-checking} classification functions separately \cite{baly_predicting_nodate}. Specifically, we stratified the original EMNLP18 dataset by political leaning and credibility, as labeled by MBFC, and analyzed the performance of 1) the full feature set, 2) individual features and 3) ablated feature sets (removing one feature type per test). Our results are summarized in~\Cref{tab:baly_ablation}. We find that, on 11 out of 12 test datasets, classifier performance using only text-based features (\texttt{articles} and \texttt{wikipedia}, derived from articles randomly sampled from the website in question, and the site's corresponding Wikipedia page, respectively) was comparable to performance on the full feature set. On five out six datasets, bias classification accuracy on text-only features actually outperformed bias classification on the whole feature set (see the bottom half of~\Cref{tab:baly_ablation}), suggesting that the full-site classifier of Baly et al. was effectively a text content classifier.
